Quick or cheap? Breaking points in dynamic markets

We examine two-sided markets where players arrive stochastically over time and are drawn from a continuum of types. The cost of matching a client and provider varies, so a social planner is faced with two contending objectives: a) to reduce players' waiting time before getting matched; and b) to form efficient pairs in order to reduce matching costs. We show that such markets are characterized by a quick-or-cheap dilemma: Under a large class of distributional assumptions, there is no 'free lunch', i.e., there exists no clearing schedule that is simultaneously optimal along both objectives. We further identify a unique breaking point signifying a stark reduction in matching cost contrasted by an increase in waiting time. Generalizing this model, we identify two regimes: one, where no free lunch exists; the other, where a window of opportunity opens to achieve a free lunch. Remarkably, greedy scheduling is never optimal in this setting.

==> 06c_microfoundations.tex <==
\delete{I tried to develop something here but suggest to delete this section again}

While the main focus of the present analysis is the trade-off  between \emph{waiting} and \emph{mismatch} from the point of view of a social planner, it is paramount to understand the micro-foundations of any proposed mechanism. For many markets with private information there do not exist ex-post efficient and budget balanced mechanisms (see \citealt{Mye83} and \citealt{Rus94}). The impossibility relies on the assumption that, with positive probability, valuations for a given 
client-provider pair are such that trade is not individually rational at any price.
We shall show that for natural preferences and strategy sets for the clients and providers our \aclp{CS} allow for an efficient mechanism, thus overcoming the usual schism.

Suppose that agents have no control over when they enter the market. This assumption is motivated by examples where the need for a good or service arises exogenously. Suppose that the match cost $w_{ij}$ can be decomposed to
\begin{equation}
w_{ij}=w_i(j)+w_j(i)
\end{equation}
such that $w_i(j), w_j(i)>0$. We assume that $w_i(j)$ ($w_j(i)$) is private information of client $i$ (provider $j$).

The action set of agent $i$ ($j$) 

Suppose that agent $i\in \mathcal C$ has utility function $u_i(w_{i}(j),b_i(j))=1-w_{i}(j)-b_i(j)$. Further, assume that agents prefer being matched earlier rather than later, as long as they derive a positive utility. We shall now set up a double-auction which will be incentive-compatible and efficient. Suppose that a given matching event the social planner opens a market place  

==> 08_thirddimension.tex <==
%----------------------------------------------------------------------
%%% OTHER EXTENSIONS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


\section{Other extensions}

\subsection{Possible extensions and interpretations}

Correlated arrival: I think that all results in Proposition \ref{maintheorem1} (need to check, and also check for other results) carry through if arrival of workers and firms is simultaneous, or, more importantly, if arrival is such that the expectation of the difference between workers and firms is lower than $|S_k|$ (the expectation in case of iid arrival). One idea is to use an urn model with delayed replacement. That would model a finite base population (of buyers and sellers) who return to the market after some time.

\cite{Ald92,Ald01} make the comment that the limit result is the same for any distribution with the same density at  $0$ since ultimately only this density matters. There is no further explanation and only the uniform distribution is mentioned as an example. Question: Can we draw edge weights independently from any distribution with the same density at $0$? Clearly the non-limit results will change. But on the other hand it will still hold that it is always optimal to choose minimal $k$-matchings. So as long as we can compute the expected minimum of a given number of possible matches we are game. This is always possible, but we shouldn't go there because notation becomes very heavy.

One could compute more accurate constants in the bounds, dependent on choice of underlying match cost distribution.

Suppose arrival time of agents to the market is a measure of whether a market place can operate efficiently. Then we can compute at what rate players arrival needs to increase to achieve constant matching and constant waiting ratio.


\subsection{Strategic considerations}

If we fix to NTU, fixed sharing rule: Note that, in particular this implies that for each player who is being matched no improvement is possible (at this particular moment in time). On the one hand, among the agents who have been matched no mutually beneficial deviation exists, since the optimal matching is stable \citep{Sha72}. On the other hand, given we assume a fixed sharing rule no agent among the unmatched is preferred by any matched agent.

If players are allowed to decline a match this will (in expectation) lead to cheaper matches in the future. So if we assume that from the moment an agent declined a match they don't count towards waiting cost anymore (i.e., no more unemployment benefits) then this is only good for us. Would this lead to us offering any type of match ?! to reduce waiting cost

\section{Why it is ok to only consider clearing schedules that match one couple at a time}

A clearing schedule at the Pareto frontier according to Lemma \ref{lem:matchcheapest} is defined by (i) the point in time when a clearing event takes place, write $f(k)$ for the function determining how many players have to be on the smaller side of the market in order for the $k^{th}$ clearing event to take place (ii) the number of players who are cleared at a given clearing event. 

Regarding (i) we shall make the assumption that $f(k)$ is non-decreasing. \textcolor{red}{argue why}
Regarding (ii) we shall make the assumption that either one couple is cleared at each clearing event or the maximal number of couples is cleared at each clearing event. The latter assumptions can be straightforwardly relaxed to a constant number of couples being cleared or the maximal number minus a constant number of couples being cleared. \textcolor{red}{argue why}

\begin{lemma} For any clearing schedule with $f(k)=\omega(\sqrt k)$ the expected matching ratio of $f_{\max}$ is $\omega (1)$.

For any clearing schedule with $f(k)=O(\sqrt k)$ the expected matching ratio is $\Omega(\log A)$. 
 \textcolor{blue}{... The expected matching ratio of $f_{\max}$ is ....  for ...}  
\end{lemma}

We shall write $\underline f_y(k)$ ($y\in [1,2,3,\ldots,f(k)]$) for the clearing schedule that matches $y$ couples at each clearing event (where $y$ may depend on $k$). For notational clarity we write  $\underline f_{\max}(k)$ instead of $ \underline f_{\underline f(k)}(k)$. Note that for given $f(k)$ the schedule that matches one couple at a time necessarily matches couples no earlier than any schedule that matches greater or equal one couple at a time. We therefore define another set of clearing schedules: Let $\overline f_y(k)$ be the clearing schedule such that the $k^th$ clearing event takes place after $k\cdot y$ couples would have been matched under the clearing schedule $\overline f_1(k\cdot y)=\underline f_1(k\cdot y)$.

\textcolor{blue}{
It is natural to assume that $f(k)$ is non-decreasing because ...\\
Further we assume that $f(k)<k$  because otherwise the proportion of matched players is not converging to one.
}
\vspace{0.5cm}

\begin{lemma} For any $f(k)$ the clearing schedule that matches exactly one couple at a time has expected matching and expected waiting ratio no larger than any other clearing schedule. For all $y\in [1,2,3,\ldots,f(k)]$:
\begin{equation}
\alpha_{f_{1}(k)} =O (\alpha_{f_y(k)}) \:\: \text{ and }\:\:  \beta_{f_{1}(k)} =O (\beta_{f_y(k)})
\end{equation}
In addition, for any clearing schedule with $f(k)=\Omega(k^{\frac{\sqrt 5 -1}{4}})$ ($\frac{\sqrt 5 -1}{4}\approx 0.31$), $f_1(k)$ is `Pareto' dominating $f_{\max}(k)$ in the following sense:
\begin{equation}
\alpha_{f_{\max}(k)} =\omega (\alpha_{f_1(k)}) \:\: \text{ and }\:\:  \beta_{f_{\max}(k)} =\Theta (\beta_{f_1(k)})
\end{equation}
\end{lemma}

\textcolor{red}{the above holds for $\gamma\leq \frac{1}{2}$ ... already something ... what can we do for the other case?}

\begin{proof}
For the first part of the Lemma, it suffices to note that matching agents earlier cannot decrease the matching costs, because any assignment chosen then can also be chosen at a later stage. In addition we need to show that the expected waiting time is not decreasing substantially (it is indeed decreasing).
\textcolor{red}{this is still missing, proof as discussed on board // maybe we need to make assumption that $f(k)\leq k$ so that the percentage number of unmatched players on market is decreasing ?}

For the second part of the Lemma, we compare the two schedules up to the point where $A$ couples are matched. For the clearing schedule that matches exactly one couple this entails $A$ clearing events. For the clearing schedule with $f_{\max}(k)=k^\gamma$ that matches the maximum number of players at each clearing event we compute the number of necessary clearing events $B$ until $A$ couples are matched
\begin{eqnarray}
\sum_1^B k^\gamma&=&A
\end{eqnarray}
Since $f(k)$ is increasing we can upper bound the lefthand side (and thus lower-bound $B$) by setting: 
\begin{eqnarray}
\int_1^{B+1} x^\gamma dx&=&A\\
\iff \frac{1}{\gamma+1}x^{\gamma+1}|_1^{B+1}&=&A\\
\iff  (B+1)^{\gamma+1}-1 &=&\frac{A}{\gamma+1}
\end{eqnarray}
From the latter equation it follows that $B=\Theta (A^{\frac{1}{\gamma+1}})$

Using Theorem \ref{Buc02,Lin04} by \cite{Buc02,Lin04} AND NOTATION AND ANALYSES FROM  PROP 4  ($S, t(\cdot,\cdot)$ and approximation thereof, Jensen's inequality) we compute the expected matching cost:
\begin{eqnarray}\label{asdfasdf}
&&\mathbb E\big [\sum_{k=1}^B\sum_{\substack{i,j\geq 0\\ i+j<k}} \frac{1}{\big (k^\gamma+|S_{t(k,k^\gamma)}|-i \big )\big(k^\gamma -j\big)}\big ]\\
&=&\sum_{k=1}^B\sum_{\substack{i,j\geq 0\\ i+j<k}} \mathbb E\big [\frac{1}{\big (k^\gamma+|S_{t(k,k^\gamma)}|-i \big )\big(k^\gamma -j\big)}\big ]\\
&>&\sum_{k=1}^B\sum_{\substack{i,j\geq 0\\ i+j<k}} \frac{1}{\big (k^\gamma+\mathbb E[|S_{t(k,k^\gamma)}|]-i \big )\big(k^\gamma -j\big)}\\
 &>&\sum_{k=1}^B\sum_{\substack{i,j\geq 0\\ i+j<k}} \frac{1}{\big (k^\gamma+\sqrt {6k}-i \big )\big(k^\gamma -j\big)}\\
 &=& \sum_{k=1}^B\sum_{\substack{i,j\geq 0\\ i+j<k\\j<k^\gamma-1}} \frac{1}{\big (k^\gamma+\sqrt {6k}-i \big )\big(k^\gamma -j\big)}+ \sum_{k=1}^B \frac{1}{k^\gamma+\sqrt {6k}}\label{asdfqwer}
\end{eqnarray}
For $\gamma \in [\frac{1}{2},1)$ we have for the rightmost sum:
\begin{eqnarray}
\sum_{k=1}^B \frac{1}{k^\gamma+\sqrt {6k} }&=&\Theta \big (\sum_{k=1}^B \frac{1}{k^\gamma} \big )\\
&=&\Theta \big (\int_{x=0}^B \frac{1}{x^\gamma}dx \big )\\
&=& \frac{1}{1-\gamma}x^{1-\gamma}|_0^B\\
&=& \frac{1}{1-\gamma}B^{1-\gamma}\\
&=&\Theta\big( A^\frac{1-\gamma}{1+\gamma} \big )
\end{eqnarray}
Thus returning to Equation \eqref{asdfasdf}, the matching ratio is lower bounded by a polynomial in $A$, this is in contrast to Proposition \ref{maintheorem1} where the matching ratio is constant for $\gamma \in (\frac{1}{2},1)$ and logarithmic for $\gamma=\frac{1}{2}$.

For $\gamma \in (\frac{\sqrt 5 -1}{4},\frac{1}{2})$ we have for the rightmost sum in Equation \eqref{asdfqwer}:
\begin{eqnarray}
\sum_{k=1}^B \frac{1}{k^\gamma+\sqrt {6k} }&=&\Theta \big (\sum_{k=1}^B \frac{1}{\sqrt k} \big )\\
&=&\Theta \big (\int_{x=0}^B \frac{1}{\sqrt x}dx \big )\\
&=& \frac{1}{2}\sqrt x|_0^B\\
&=& \frac{1}{2}\sqrt B\\
&=&\Theta\big( A^\frac{1}{2(1+\gamma)} \big )
\end{eqnarray}
Thus returning to Equation \eqref{asdfasdf}, the matching ratio is lower bounded by $ A^\frac{1}{2(1+\gamma)}$. From Proposition \ref{maintheorem1}$(CS_{0<\gamma<\frac{1}{2}})$ we know that $\alpha_{f_1(k)}=O(A^{1-2\gamma})$. Thus a sufficient condition for $\alpha_{f_{\max}(k)}=\omega (\alpha_{f_1(k)})$ is:
\begin{eqnarray}
A^\frac{1}{2(1+\gamma)}&=&\omega (A^{1-2\gamma})\\
\iff \frac{1}{2(1+\gamma)} &>&{1-2\gamma}\\
\iff 4\gamma^2+2\gamma-1 &>&0
\end{eqnarray}
The latter quadratic equation has one negative solution and the solution $\frac{\sqrt 5 -1}{4}$ and thus the result follows.
\end{proof}



==> 99_dump.tex <==


%\fi



%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\if{false}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\section{results we don't need to restate}

\begin{theorem}[\citealt{Buc02,Lin04}] \label{Buc02,Lin04}
Consider the minimum weight matching and suppose that $w_{ij}\sim exp(1)$ iid. The expected matching cost of the minimum $k$-assignment  in a market with $\mathcal B, \mathcal S \geq k$ is:
\begin{equation}
 \sum_{\substack{i,j\geq 0\\ i+j <k}}\frac{1}{(N_\mathcal B-i)\cdot (N_\mathcal S-j)}
\end{equation}
\end{theorem}

\vspace{0.5cm}

\begin{theorem}[\citealt{Ald01}]\label{Ald01}
Let $N_\mathcal{B}=N_\mathcal{S}=N$ and suppose that $w_{ij}\sim \exp(1)$ iid. The expected matching cost for the minimum perfect matching approaches $\frac{\pi^2}{6}$ from below.
\end{theorem}

\vspace{0.5cm}

\begin{theorem}[\citealt{Wae05}]\label{Wae05}
Suppose that $w_{ij}\sim \exp(\lambda_{ij})$ where $\lambda_{ij}=\lambda^{\mathcal B}_i\cdot \lambda^{\mathcal S}_j$.  The expected matching cost of the minimum $k$-assignment  in a market with $\mathcal B, \mathcal S \geq k$ is:
\begin{equation}\label{generalformulae}
 \sum_{I,J} {N_{\mathcal B}+N_{\mathcal S}-1-|I|-|J|\choose k-1-|I|-|J|}\frac{(-1)^{k-1-|I|-|J|}}{\big (\sum_{i\notin I}\lambda^{\mathcal B}_i\big )\cdot \big(\sum_{j\notin J}\lambda^{\mathcal S}_j\big )}
\end{equation}
where the summation is over sets $I\subset \{1,2,\ldots N_{\mathcal B}\}$ and $I\subset \{1,2,\ldots N_{\mathcal S}\}$ such that $|I|+|J|<k$.
\end{theorem}

We note that for $k=1$ Equation \eqref{generalformulae} simplifies to:
\begin{equation}
\frac{1}{\big (\sum_{i\notin I}\lambda^{\mathcal B}_i\big )\cdot \big(\sum_{j\notin J}\lambda^{\mathcal S}_j\big )}
\end{equation}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%

\section{Possible extensions}

\cite{Lin00} conjecture (later proved by \cite{Wae05}) an exact formula for a $k$ assignment for assignment games where match weights are either zero (cost)  or from $\exp(1)$ distributions. This constitutes the existence of ``perfect'' matches. Not so interesting.


One neat idea is to turn it around into profit per edge. Then we could discount profits with a common discounting factor, $e^{-\delta t}$. The distribution of edge weights then would be of the form:
\begin{equation}
f(x,\lambda)=\begin{cases} \lambda e^{\lambda (x-c)} \:\:\: x\leq  c \\ 0  \:\:\: else \end{cases}
\end{equation}

%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%

\subsection{One side is waiting in the market}

\begin{proposition}
Suppose that one side of the market is already there and the other side arrives over time (and $|\mathcal B|=|\mathcal S|=n$). 
\begin{enumerate}[(i)]
\item The greedy clearing schedule has expected matching ratio of $\log (n)$. 
\item The patient clearing schedule has expected matching ratio of $c\leq \frac{\pi^2}{6}$.
\end{enumerate}
\end{proposition}
	
\begin{proof}
(i) via harmonic series

(ii) \cite{Ald01}
\end{proof}

%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%

\begin{proposition}\label{th_waitintime}The expected waiting ratio for the different clearing schedules is given by:
\begin{enumerate}[(i)]
\item[(ii/iii)] The greedy and FIFO clearing schedules have an expected waiting cost of $\beta(N)=\sum_{k=1}^N t(k,1)=\Theta(N^2)$.
\item[(iv)] The clearing schedule that matches exactly one couple when $C$ buyers and sellers are currently in the market  has an expected waiting ratio of $\beta(N)=2$ for $N$ large enough.
\item[(v-vii)] The clearing schedule that matches the $k^{th}$ couple when $k^\gamma$ buyers and sellers are currently in the market has an expected waiting ratio of $\beta(N)=O(1)$.
\end{enumerate}
\end{proposition}

\begin{proof}[Proof of Proposition \ref{th_waitintime}.] Let $\tau(k)$ be the moment the $k^{th}$ couple is matched (given a particular clearing schedule). 

(ii/iii) The greedy clearing schedule has an expected waiting time equivalent to the arrival times of players, by the independence of the arrival times of players, and the expected arrival times being at distance $1$:
\begin{eqnarray}
\mathbb E [\sum_{k=1}^N \tau(k)]&=&\sum_{k=1}^N \mathbb E [\tau(k)]\\
&=&\sum_{k=1}^N \tau(t(k,1))\\
&\in&[\sum_{k=1}^N \tau(2k),\sum_{k=1}^N \tau(4k)]
\end{eqnarray}
where for the last two lines note first that the arguments of the summands are bounded below by $2k$ and by  Equation \eqref{eqhelpeq} in the proof of Proposition \ref{maintheorem1} they are bounded above by $4k$. Second, note that, the expected time between the arrival of two agents is $1$.
This concludes the proof of the waiting time in the optimal schedule (w.r.t. waiting time).

(iv) Let $\tau(t(0,1))=0$. Then with the same reasoning as above and the reformulation of $t(k,C)$ as in the proof of  Proposition \ref{maintheorem1} we have:
\begin{eqnarray}
\beta(N)&=&\frac{\sum_{k=1}^N \tau(t(k,C))}{\sum_{k=1}^N \tau(t(k,1))}\\
&=& \frac{\sum_{k=1}^N \tau(t(1,C))+\tau(t(k-1,1))}{\sum_{k=1}^N \tau(t(k,1))}\\
&<& \frac{\sum_{k=1}^N \tau(t(C,1))+\tau(t(k,1))}{\sum_{k=1}^N \tau(t(k,1))}
\end{eqnarray}
Next note that $t(k,1)$ is strictly increasing in $k$. Thus there exists $N^*$ such that for $N>N^*$ we have:
\begin{eqnarray}
\frac{\sum_{k=1}^N \tau(t(C,1))+\tau(t(k,1))}{\sum_{k=1}^N \tau(t(k,1))}&<&\frac{\sum_{k=1}^N 2\tau(t(k,1))}{\sum_{k=1}^N \tau(t(k,1))}=2
\end{eqnarray}
Thus the expected waiting ratio $\beta$ is bounded above by $2$.

(v-vii) As above we consider:
\begin{eqnarray}
\beta(N)&=&\frac{\sum_{k=1}^N \tau(t(k,k^\gamma))}{\sum_{k=1}^N \tau(t(k,1))}\end{eqnarray}
Note that the summands in the denominator are trivially bounded below by $2k$. 
For the numerator first note that $t(k,k^\gamma)=t(k+k^\gamma,1)$. Thus by Equation \eqref{eqhelpeq} in the proof of Proposition \ref{maintheorem1} we have that the summands in the numerator are bounded above by $4(k+k^{\gamma})$. Given $\gamma\in (0,1)$ we have:
\begin{eqnarray}
\beta(N)&<&\frac{\overbrace{\sum_{k=1}^N 4(k+k^{\gamma})}^{=O(N^{2})}}{\underbrace{\sum_{k=1}^N 2k}_{+o(N^2)}}=O(1)
\end{eqnarray}
where the bound on the numerator and denominator follow from the Euler-Maclaurin formula.
Thus the expected waiting ratio $\beta$ is  $O(1)$.

\end{proof}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%

\section{Envisioned results}

In addition to a player's payoff from matching, suppose that there is a cost for waiting in the market. For a player who arrived in the market at time $\tau_0$ and who is being matched (and thus leaves the market) at time $\tau_1$ suppose that the cost is given by a function $c(\tau_1-\tau_0)$. We shall consider the cost to be either additively separable or multiplicative.

\begin{theorem}
Suppose that the cost function $c$ is of form [...], match values are drawn iid from the $exp(1)$ distribution and players arrival clocks are iid.
The optimal clearing schedule is [...].
\end{theorem}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\section{trying out stuff}

\subsection{tight bound for Proposition 3 (iii)}

suppose that k is even (for ease of exposition)
{\footnotesize
\begin{eqnarray}
&&\mathbb E[\frac{1}{|S_k|+1}]\\
&=&\sum_{i=0}^k {k\choose i} \frac{1}{2^k}\cdot \frac{1}{|2i-k|+1}\\
&=& \frac{1}{2^k} \sum_{i=0}^k \frac{k!}{i!(k-i)!} \frac{1}{|2i-k|+1}\\
&=& \frac{1}{2^k} \sum_{i=0}^{k/2-1} \frac{k!}{i!(k-i)!} \frac{1}{k-2i+1}+\frac{1}{2^k} \sum_{i=k/2+1}^k \frac{k!}{i!(k-i)!} \frac{1}{2i-k+1}+\frac{1}{2^k}\frac{k!}{ ((\frac{1}{2}k)!)^2}\\
&=& \frac{2}{2^k}\sum_{i=0}^{k/2-1} \frac{k!}{i!(k-i)!} \frac{1}{k-2i+1}+\frac{1}{2^k}\frac{k!}{ ((\frac{1}{2}k)!)^2}\\
&=& \frac{2}{2^k}\sum_{i=0}^{k/2-1} \frac{k\cdot (k-1)\cdot \ldots (k-i+1)}{i\cdot (i-1)\ldots 1} \frac{1}{k-2i+1}+\frac{1}{2^k}\frac{k!}{ ((\frac{1}{2}k)!)^2}\\
&=& \frac{2}{2^k}\big [\frac{1}{k+1}+\frac{k}{k-1}+\frac{k(k-1)}{2(k-3)}+\frac{k(k-1)(k-2)}{6(k-5)}+\ldots+
\frac{k(k-1)(k-2)\ldots(\frac{k}{2}+2)}{(\frac{k}{2}-1)(\frac{k}{2}-2)\ldots 2 \cdot 3}     \big ]\\
&&+\frac{1}{2^k}\frac{k!}{ ((\frac{1}{2}k)!)^2}
\end{eqnarray}
}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\fi


==> Test.tex <==
\emph{This is a test.}
In this paper,
we examine a class of \emph{online assignment games}
that are induced by the stochastic arrival of market participants in a heterogeneous two-sided market.
